Bicriteria Approximation Algorithms for the Submodular Cover Problem

In this paper, we consider the optimization problem Submodular Cover (SCP), which is to find a minimum cardinality subset of a finite universe $U$ such that the value of a submodular function $f$ is above an input threshold $\tau$. In particular, we consider several variants of SCP including the general case, the case where $f$ is additionally assumed to be monotone, and finally the case where $f$ is a regularized monotone submodular function. Our most significant contributions are that: (i) We propose a scalable algorithm for monotone SCP that achieves nearly the same approximation guarantees as the standard greedy algorithm in significantly faster time; (ii) We are the first to develop an algorithm for general SCP that achieves a solution arbitrarily close to being feasible; and finally (iii) we are the first to develop algorithms for regularized SCP. Our algorithms are then demonstrated to be effective in an extensive experimental section on data summarization and graph cut, two applications of SCP.

==> Sections/Old/Cover.tex <==




\begin{algorithm}
% \label{alg:sg}
\begin{algorithmic}[1]

\Procedure{\texttt{KSC-Stream}}{$\tau$}
  \State {\bfseries{Input: }$\tau$, $\delta\in(0,1)$}
  \State{ $S_{-1}\gets\emptyset$, $r\gets-1$}
  \While{$f(S_r)<\alpha\tau$}
  \State $r\gets r+1$
  \State $OPT_r=(1+\delta)^rc_{min}$
        \State {$S_r\gets$\texttt{KSM-Stream}($OPT_r$)}
  \EndWhile
  \State \textbf{return} $S$
\EndProcedure

\end{algorithmic}
\end{algorithm}
In particular, notice that the when the cardinality constraint parameter $\kappa$ increases, the size of subset sampled at each iteration in stochastic greedy algorithm  decreases. This motivates the new algorithm. By using samples and results obtained in the case where guess of OPT is small, we can further reduce the sample complexity. 
The algorithm is given in Algorithm \ref{alg:stoc_cover}.

% There are two choices of $OPT_r$ in the algorithm. If we choose to utilize the previous result as in the converting algorithm above, the choice of $OPT_r:=\max\{(1+\frac{\epsilon}{3})^t|(1+\frac{\epsilon}{3})^t\ln(3/\epsilon)\leq r\}$. The sample complexity is then $O(\frac{n\ln(OPT)\ln^2(3/\epsilon)3/\epsilon}{\ln(1+3/\epsilon)})$. We defer the proof and calculation to the appendix. Here we present the analysis in the case where $OPT_r=\lfloor\frac{r-1}{\ln(3/\epsilon)}\rfloor$. 





Hence, Algorithm \ref{alg:stoc_cover} improves both the theoretical approximation guarantee and also the sample complexity.\\

Should talk about how you can't have a single pass cover algorithm.s

\begin{theorem}
    Any streaming $(\alpha,\beta)$-bicriteria approximation algorithm for KSM that runs in 
    $\mathcal{P}(n)$ passes and requires space usage of 
    $\mathcal{M}(n)$ can be converted into a $(\beta,\alpha)$-bicriteria approximation algorithm for KSC that runs in 
    $O((\log\frac{OPT}{\cmin})\mathcal{P}(n))$ passes and requires space usage of 
    $\mathcal{M}(n)$. Here $OPT_\tau$ is the optimal value of $KSC(\tau)$.
\end{theorem}
\begin{proof}
{\color{blue}Might need some proofs about $\cmin$ here.}  When $OPT_r$ increases and falls into the range that $c(S^*)\leq OPT_r \leq(1+\delta)c(S^*)$, we have that
\begin{align*}
    f(S_r)&\geq\alpha\max\{f(S):c(S)\leq OPT_r\}\\
    &\geq\alpha\max\{f(S):c(S)\leq c(S^*)\}\geq\alpha\tau,
\end{align*}
where the last inequality follows from Lemma \ref{lem:dual_opt}. Besides, we have
\begin{align*}
    c(S_r)\leq\beta OPT_r\leq \beta(1+\delta)c(S^*)
\end{align*}
Define $r_0$ to be $r_0=1+\frac{\log(c(S^*)/\cmin)}{\log{1+\delta}}$. It follows that $C_{r_0}=\cmin(1+\delta)^{r_0}\geq (1+\delta)c(S^*)$. Thus the algorithm stops before $r=r_0$. 
\end{proof}

TODO: Possibility of making parallel guesses of the optimal solution instead of multipass.

Now regularized objectives. But how do we know if $\tau$ is feasible? Notice that one difficulty we have to overcome is how to check the guarantee for the stopping condition of cover.




==> Sections/Old/DistortedGreedy.tex <==
In this subsection, we study the Regularized Submodular Maximization problem with Cardinality constraint, i.e., $\argmax\{f(X)- c(X): |X|\leq \kappa\}$. Here $c$ is a monotone linear function. 
First, an approach inspired by that of \cite{harshaw2019submodular} is taken.
A greedy algorithm (\distgreed) is employed where instead of
the max marginal gain to $g-c$ being used to pick the element, the $i$th element is
chosen by using a distorted objective, $\Phi_i$.

\begin{paragraph}{Definitions}
  (i) Let $\beta\in[0,1]$ be given. Define the $i$th distorted version of $g-c$ to be
  \begin{align*}
    \Phi_i(X) = \left(1-\frac{1}{\kappa}\right)^{t-i}g(X) - \beta c(X)
  \end{align*}
  where $t=\ln(1/\epsilon)\kappa$.
  (ii) Define $S_i$ to be $S$ after the $i$th iteration of the while loop in
  \distgreed.
  For $i$ is greater than the number of iterations that \distgreed took, then
  $S_i$ is just the final value of $S$.
  $s_i$ is the element added to $S$ during the $i$th iteration,
  if such an element exists.
\end{paragraph}


\begin{algorithm}
\label{distortedgreedy}
\begin{algorithmic}[1]

\Procedure{\distgreed}{$\epsilon, \tau$, $\kappa$}
  \State $S\gets\emptyset$
  \State $i\gets 1$
  \While{$|S|<\ln(1/\epsilon)\kappa$}
    \State $u\gets\argmax_{x\in U}\Delta \Phi_i(S,x)$
    \If{$\Delta \Phi_i(S,x) > 0$}
      \State $S\gets S\cup\{u\}$
      \State $i\gets i+1$
    \Else
      \State \textbf{break}
    \EndIf
  \EndWhile
  \State \textbf{return} $S$
\EndProcedure

\end{algorithmic}
\end{algorithm}

\begin{lemma}
  \label{distlemma}
  Let $i+1$ be an iteration of the while loop in \distgreed. Then
  \begin{align*}
    \Phi_{i+1}(S_{i+1})-\Phi_{i}(S_i) \geq
    \frac{1}{\kappa}\left(1-\frac{1}{\kappa}\right)^{t-(i+1)}g(S^*)-\beta\frac{c(S^*)}{\kappa}.
  \end{align*}
\end{lemma}
\begin{proof}
  TODO: Case where nothing was added.
  Now, suppose that during iteration $i+1$ an element was added to $S$.
  First, notice that
  \begin{align*}
    \Phi_{i+1}(S_{i+1})-\Phi_i(S_i) & =\Phi_{i+1}(S_{i+1})-\Phi_{i+1}(S_i)+\Phi_{i+1}(S_{i})-\Phi_i(S_i)\\
    %= \left(1-\frac{1}{\kappa}\right)^{t-(i+1)}g(S_{i+1})-\beta c(S_{i+1})
    %- \left(1-\frac{1}{\kappa}\right)^{t-i}g(S_i)+\beta c(S_i) \\
    % &= \left(g(S_{i+1} - \left(1-\frac{1}{\kappa}\right)g(S_i)\right)\left(1-\frac{1}{\kappa}\right)^{t-(i+1)}
       % -\beta c(s_{i+1}) \\
    &= \Delta\Phi_{i+1}(S_i,s_{i+1})
       + \frac{1}{\kappa}\left(1-\frac{1}{\kappa}\right)^{t-(i+1)}g(S_i).
  \end{align*}
  In addition, notice that
  \begin{align*}
    %\left(1-\frac{1}{\kappa}\right)^{t-(i+1)}\Delta g(S_i,s_{i+1}) - \beta c(s_{i+1})
     \Delta \Phi_{i+1} (S_i,s_{i+1}) &\overset{(a)}{\geq} \frac{1}{\kappa}\sum_{o\in S^*}\left(\Delta \Phi_{i+1} (S_i,s_{i+1}) \right) \\
    &\geq \frac{1}{\kappa}\sum_{o\in S^*}\left(\left(1-\frac{1}{\kappa}\right)^{t-(i+1)}\Delta g(S_i,o)-\beta c(o)\right) \\
    &= \frac{1}{\kappa}\left(1-\frac{1}{\kappa}\right)^{t-(i+1)}\sum_{o\in S^*}\Delta g(S_i,o)-\beta \frac{c(S^*)}{\kappa}\\
    &\overset{(b)}{\geq}\frac{1}{\kappa}\left(1-\frac{1}{\kappa}\right)^{t-(i+1)}\left(g(S_i\cup S^*)-g(S_i)\right)-\beta \frac{c(S^*)}{\kappa}\\
    &\overset{(c)}{\geq}\frac{1}{\kappa}\left(1-\frac{1}{\kappa}\right)^{t-(i+1)}\left(g(S^*)-g(S_i)\right)-\beta \frac{c(S^*)}{\kappa}
  \end{align*}
  where (a) is because of the greedy choice of $s_i$; (b) is by the submodularity of
  $g$; and (c) is by the monotonicity of $g$.
  Combining the previous two equations gives the result of Lemma \ref{distlemma}.
\end{proof}

\begin{theorem}
  \label{distthm}
  \distgreed produces a solution $S$ such that $|S|\leq\ln(1/\epsilon)\kappa$ and
  \begin{align*}
    g(S)-\beta c(S)\geq (1-\epsilon)g(S^*)-\beta \ln(1/\epsilon)c(S^*).
  \end{align*}
\end{theorem}
\begin{proof}
  We will use Lemma \ref{distlemma} to prove Theorem \ref{distthm}.
  See that
  \begin{align*}
    g(S)-\beta c(S) &\overset{(a)}{\geq} \Phi_t(S_t) - \Phi_0(S_0) \\
    &= \sum_{i=0}^{t-1}\left(\Phi_{i+1}(S_{i+1})-\Phi_i(S_i)\right) \\
    &\overset{(b)}{\geq} \sum_{i=0}^{t-1}\left(\frac{1}{\kappa}\left(1-\frac{1}{\kappa}\right)^{t-(i+1)}g(S^*)-\beta \frac{c(S^*)}{\kappa}\right)\\
    &= \frac{g(S^*)}{\kappa}\sum_{i=0}^{t-1}\left(1-\frac{1}{\kappa}\right)^{t-(i+1)}-\beta \ln\left(1/\epsilon\right)c(S^*)\\
    &= \frac{g(S^*)}{\kappa}\sum_{i=0}^{t-1}\left(1-\frac{1}{\kappa}\right)^i-\beta \ln\left(1/\epsilon\right)c(S^*)\\
    &\overset{(c)}{=} \left(1-\left(1-\frac{1}{\kappa}\right)^t\right)g(S^*)-\beta \ln\left(1/\epsilon\right)c(S^*)\\
    &\geq(1-\epsilon)g(S^*)-\beta \ln\left(1/\epsilon\right)c(S^*)
  \end{align*}
  where (a) is because $g(\emptyset)\geq 0$;
  (b) is because Lemma \ref{distlemma};
  and (c) is by the formula for geometric series.

\end{proof}


==> Sections/Old/DistortedGreedy2.tex <==




In this subsection, another distorted-greedy algorithm is described here. First, we assume that the only $OPT$ is known. A greedy algorithm (\texttt{distorted-greedy-1}) is proposed here. 

\begin{algorithm}
\label{distortedgreedy1}
\begin{algorithmic}[1]

\Procedure{\texttt{distorted-greedy-1}}{$\epsilon, \tau$, $|OPT|$}
  \State $S\gets\emptyset$
  \State $i\gets 1$
  \While{$|S|<\ln(1/\epsilon)|OPT|$}
    \State $u\gets\argmax_{x\in U}(1-\frac{1}{|OPT|})^{t-i}\Delta g(S,x)-\frac{1-\epsilon}{\ln(1/\epsilon)}\Delta c(S,x)$
      \State $S\gets S\cup\{u\}$
      \State $i\gets i+1$
  \EndWhile
  \State \textbf{return} $S$
\EndProcedure

\end{algorithmic}
\end{algorithm}

\begin{theorem}
  \label{distthm1}
  \texttt{distorted-greedy-1} produces a solution $S$ such that $|S|\leq\ln(1/\epsilon)|OPT|$ and
  \begin{align*}
    g(S)-\frac{1-\epsilon}{\ln(1/\epsilon)}c(S)\geq (1-\epsilon)(g(OPT)-c(OPT)).
  \end{align*}
\end{theorem}

% \begin{proof}{proof sketch}
% \end{proof}
\proofsketch
Denote $S_i$ to be $S$ before the $i$-th iteration, and $u_i$ to be the item picked at step $i$. Then from the greedy strategy, we have that for any item $u\in S^*$, we have
\begin{align*}
    (1-\frac{1}{k})^{t-i}\Delta g(S_i,u_i)-\frac{1-\epsilon}{\ln(1/\epsilon)}\Delta c(S_i,u_i)\geq(1-\frac{1}{k})^{t-i}\Delta g(S_i,u)-\frac{1-\epsilon}{\ln(1/\epsilon)}\Delta c(S_i,u)
\end{align*}
Because $g$ is submodular and $c$ is supermodular, we have
\begin{align*}
    (1-\frac{1}{k})^{t-i}\Delta g(S_i,u_i)-\frac{1-\epsilon}{\ln(1/\epsilon)}\Delta c(S_i,u_i)\geq\frac{(1-\frac{1}{k})^{t-i}[ g(S_i\cup S^*)-g(S_i)]-
    \frac{1-\epsilon}{\ln(1/\epsilon)} [c(S_i\cup S^*)-c(S_i)]}{k}
\end{align*}
Since $g$ and $c$ is monotone and $c$ is submodular, it follows that
\begin{align*}
    (1-\frac{1}{k})^{t-i}\Delta g(S_i,u_i)-\frac{1-\epsilon}{\ln(1/\epsilon)}\Delta c(S_i,u_i)\geq\frac{(1-\frac{1}{k})^{t-i}[ g( S^*)-g(S_i)]-
    \frac{1-\epsilon}{\ln(1/\epsilon)} [c( S^*)]}{k}.
\end{align*}
By some calculation, we have that
\begin{align*}
    (1-\frac{1}{k})^{t-i}g(S_{i+1})-\frac{1-\epsilon}{\ln(1/\epsilon)} c(S_{i+1})\geq(1-\frac{1}{k})^{t-i+1}[ g(S_i)]-\frac{1-\epsilon}{\ln(1/\epsilon)} [c( S_i)]+\frac{1}{k}(1-\frac{1}{k})^{t-i}g( S^*)-
    \frac{1-\epsilon}{k\ln(1/\epsilon)} [c( S^*)].
\end{align*}
Denote $f(i)=(1-\frac{1}{k})^{t-i+1}[ g(S_i)]-\frac{1-\epsilon}{\ln(1/\epsilon)} [c( S_i)]$, then it follows that
\begin{align*}
    f(i+1)\geq f(i)+\frac{1}{k}(1-\frac{1}{k})^{t-i}g( S^*)-
    \frac{1-\epsilon}{k\ln(1/\epsilon)} [c( S^*)].
\end{align*}
By induction, we have that
\begin{align*}
    f(t+1)&\geq \sum_{i=1} ^{t}\frac{1}{k}(1-\frac{1}{k})^{t-i}g( S^*)-
    \frac{1-\epsilon}{k\ln(1/\epsilon)} [c( S^*)]\\
    &\geq(1-\epsilon) ({g(S^*)-c(S^*)})
\end{align*}

==> Sections/Old/DistortedStreaming.tex <==

\begin{algorithm}
\label{distortedstream}
\begin{algorithmic}[1]

\Procedure{\diststrm}{$\epsilon, \beta, |OPT|$}
  \State $S\gets\emptyset$
  \While {$|S|<|OPT|/\epsilon$ and $u\gets stream$}
    \If {$\Delta g(S,u)-\beta c(u)\geq\epsilon\tau/|OPT|$}
      \State $S\gets S\cup\{u\}$
    \EndIf
  \EndWhile
  \State \textbf{return} $S$
\EndProcedure

\end{algorithmic}
\end{algorithm}

\begin{theorem}
  \label{diststrmthm}
  Suppose input $\beta\geq 1$.
  \diststrm produces a solution $S$ such that $|S|\leq|OPT|/\epsilon$ and
  \begin{align*}
    g(S)-c(S)\geq (1-1/\beta-\epsilon(1-1/\beta))g(OPT)-(\beta+1-\epsilon(1-1/\beta))c(OPT).
  \end{align*}
  In particular, if $\beta=1/\epsilon$,
  \begin{align*}
    %g(S)-c(S)\geq (1-2\epsilon+\epsilon^2)g(OPT)-(1/\epsilon+1-\epsilon + \epsilon^2)c(OPT).
    g(S)-c(S)\geq (1-\epsilon)^2g(OPT)-(1/\epsilon-\epsilon + \epsilon^2+1)c(OPT).
  \end{align*}
\end{theorem}
\begin{proof}
  First, consider the case where at the end of \diststrm $|S|=|OPT|/\epsilon$.
  Then,
  \begin{align*}
    g(S)-c(S) &\overset{(a)}{\geq} g(S)-g(\emptyset)-\beta c(S)\\
    &\overset{(b)}{\geq} \sum_{i=1}^{|S|}\left(\Delta g(S_{i-1},s_i)-\beta c(s_i)\right)\\
    &\overset{(c)}{\geq} |S|\epsilon\tau/|OPT|\\
    &\overset{(d)}{=} \tau\\
    &\geq g(OPT)-c(OPT).
  \end{align*}
  where (a) is because $\beta\geq 1$ and $g(\emptyset)\geq 0$;
  (b) is by submodularity of $g$;
  (c) is by the condition of adding an element to $S$;
  and (d) is by the assumption that $|S|=|OPT|/\epsilon$.

  Next, consider the case where at the end of \diststrm $|S|<|OPT|/\epsilon$.
  Then see that
  \begin{align}
    \label{eqn1}
    g(OPT)-g(S)-\beta c(OPT) &\overset{(a)}{\leq} g(OPT\cup S)-g(S)-\beta c(OPT)\nonumber\\
    &\overset{(b)}{\leq} \sum_{o\in OPT}\left(\Delta g(S,o)-\beta c(o)\right)\nonumber\\
    &\overset{(c)}{<} \epsilon\tau
  \end{align}
  where (a) is due to the monotonicity of $g$;
  (b) is due to submodularity of $g$;
  and (c) is due to submodularity combined with the fact that any element of
  $OPT$ is either in $S$ or had been rejected.

  In addition,
  \begin{align}
    \label{eqn2}
    g(S) - \beta c(S) &\overset{(a)}{\geq} g(S)-g(\emptyset)-\beta c(S)\nonumber \\
    &\overset{(b)}{\geq} \sum_{i=1}^{|S|}\left(\Delta g(S_{i-1},s_i)-\beta c(s_i)\right)\nonumber \\
    &\overset{(c)}{\geq} |S|\epsilon\tau/|OPT|\nonumber\\
    &\geq 0
  \end{align}
  where (a) is because $g(\emptyset)\geq 0$;
  (b) is by submodularity of $g$;
  and (c) is by the condition to add elements to $S$.

  Finally, we have that
  \begin{align*}
    g(S)-c(S) &\overset{(a)}{\geq} (1-1/\beta)g(S)\\
    &\overset{(b)}{\geq} (1-1/\beta)\left(g(OPT)-\beta c(OPT)-\epsilon\tau\right)\\
    &= (1-1/\beta)g(OPT)-(\beta+1)c(OPT)-(1-1/\beta)\epsilon\tau\\
    &\overset{(c)}{\geq}(1-1/\beta-\epsilon(1-1/\beta))g(OPT)-(\beta+1-\epsilon(1-1/\beta))c(OPT)
  \end{align*}
  where (a) is by Inequality \ref{eqn2};
  and (b) is by Inequality \ref{eqn1};
  and (c) is because $g(OPT)-c(OPT)\geq\tau$.
\end{proof}


==> Sections/Old/Monotone.tex <==
\begin{subsection}{Monotone submodular cover}
\label{section:monotone_objectives}
In this section, we consider \scp where there is the additional assumption that the submodular function $f$ is monotone. The analogous version of \smp is well-known to be approximated by the standard greedy algorithm with a guarantee of $1-1/e$ \citep{nemhauser1978analysis}. It turns out, because the objective $f$ is monotone several greedy algorithms can simply ``keep going'' and achieve $f$ value arbitrarily close to that of the optimal solution. 
Because the objective is monotone, it is clear that if we keep adding elements we must eventually reach an $f$ value of $OPT$. It turns out that by greedily choosing at most $\ln(1/\epsilon)|OPT|$ elements we can ensure that we are at least $(1-\epsilon)\tau$. Therefore by running the greedy algorithm until $f$ reaches $(1-\epsilon)\tau$ we have a bicriteria approximation guarantee for \scp. Further, this guarantee is tight in the sense that there exist instances of \scp such that the greedy algorithm must take about this many in order to ensure that we are at least $(1-\epsilon)\tau$. A similar result also holds for the faster threshold greedy algorithm of \cite{badanidiyuru2014fast}. These facts are stated in the following theorem and proven in the appendix.

\begin{theorem}
\label{thm:greedy_and_threshold_greedy}
    The following bicriteria approximation algorithms exist for \scp:
    \begin{itemize}[noitemsep]
        \item[(i)] For any $\epsilon\in(0,1)$, \greedybi is a $(\ln(1/\epsilon), 1-\epsilon)$-bicriteria approximation algorithm for \scp that takes time $O(n\ln(1/\epsilon)|OPT|)$. Further, there exists an instance of \scp where the greedy algorithm must add at least $\log_{1-1/|OPT|}(\epsilon)/|OPT|$ in order for the $f$ value to reach a factor of $1-\epsilon$.
        \item[(ii)] Threshold greedy result.
        %\item[(iii)] \stream produces a solution with $(1-\epsilon,1/\epsilon)$-bicriteria approximation guarantee to SM in a single query of $f$ per arriving element, TODO memory, and a single pass through $U$.
    \end{itemize}
\end{theorem}
%It is not just the greedy algorithm that can get arbitrarily close to $f(OPT)$ by expanding beyond the budget $\kappa$. A similar result can be gotten for many other existing algorithms for \smp with a monotone objective. However, unlike the greedy algorithm it is typically the case that one must modify the algorithm further than simply expanding the budget. For example, a similar result can be gotten for the scalable greedy algorithm \sgbi \citep{mirzasoleiman2015lazier} by adding $O(\ln(1/\epsilon)$ times as many elements as the budget, but on the other hand we must adjust the random sampling to take more samples at each step to account for the size of the optimal solution being relatively small compared to the returned solution. A further discussion of how \sgbi and a number of other existing algorithms can be transformed into bicriteria ones in given in the appendix. We formalize our results for both the standard greedy algorithm and the stochastic greedy algorithm below.

On a related note, it is easy to show using the same analysis that for an instance of \smp if we add greedily add $\ln(1/\epsilon)\kappa$ elements then we have a $(1-\epsilon, \ln(1/\epsilon))$-bicriteria guarantee for \smp. The above algorithms are superior compared to using the converting technique with the bicriteria algorithm for \smp because they result in many less queries of $f$ and give identical results. In particular, each time we guess increasing $\kappa$ we make the same greedy sequence. 

An important additional algorithm is \sgbi of \citep{mirzasoleiman2015lazier}. In \sgbi, a random sample of $U$ is taken at each greedy step and the element of highest marginal gain within this set is chosen. Unlike the algorithms presented above, we cannot simply take \sgbi and ``keep going''. This is because of two reasons: (i) We do not know the size of the optimal solution $|OPT|$ which is important in deciding how many samples to take at each step; (ii) The guarantee on $f$ in expectation so we cannot simply keep checking whether $f$ is sufficiently close to $\tau$ as the stopping condition. While it is possible to keep guessing $OPT$, and then running \sg for \smp sufficiently many times to convert to a guarantee w.h.p. (as is done in Section \ref{section:nonmono}), this results in many wasteful queries of $f$. For the remainder of the section, we focus on presenting a new algorithm that can be viewed as analogous to \sg but for \scp.

\begin{subsubsection}{Stochastic greedy algorithm for \scp}
\input{graphs/greedy}
The algorithm \sgbi is a scalable algorithm for \scp that runs in time TODO if $\epsilon$ is constant. \sgbi keeps track of $O(\ln(1/\delta))$ solutions. At each iteration, a random sample of $U$ is taken independently for each solution and the element from the sample with highest marginal gain is added to the corresponding solution. At first, the greedy steps are near exact but the number of samples decreases after each iteration. This is because the number of samples must be proportional to $|OPT|$. In particular, the smaller $|OPT|$ the more samples we need. While we do not know $|OPT|$ exactly, the longer \sgbi runs without any of the solutions reaching $(1-\epsilon)\tau$ then the larger $|OPT|$ must be, which corresponds to less needed samples. The reason we need so many solutions is because we want to be able to say that at least one of their $f$ values will have reached $(1-\epsilon)\tau$. Overall, \sgbi needs more queries of $f$ by a factor of TODO compared to \sg. Pseudocode for \sgbi is presented in Algorithm \ref{alg:stoc_cover}. 

\begin{algorithm}
\caption{\stocover}\label{alg:stoc_cover}
\textbf{Input}: $\epsilon,\tau$\\
\textbf{Output}: $S\subseteq U$
\begin{algorithmic}[1]
    \State $S_i\gets \emptyset$ $\forall i\in\left\{1,...,\ln(1/\delta)/\ln(2)\right\}$
  \State $r\gets 1$
  \While {$f(S_i) < (1-\epsilon)\tau$ $\forall i$}
    \For {$i\in\left\{1,...,\ln(1/\delta)/\ln(2)\right\}$}
        \State $R\gets$ sample $\min\{n, n\ln(3/\epsilon)/\lfloor r/\ln(3/\epsilon)+1\rfloor\}$ elements from $U$
        \State $u\gets\argmax_{x\in R}\Delta f_\tau(S_{j},x)$
        \State $S_j\gets S_j\cup\{u\}$
    \EndFor
    \State{$r\gets r+1$}
    % \If{ $\frac{\sum_{j=1}^Nf_\tau(S^{(j)})}{N} \geq(1-\epsilon)\tau$}\label{line:full}
    %      \State \textbf{break}
    %      \EndIf
  \EndWhile
  \State \textbf{return} $\argmin\{|S_i|: f(S_i)\geq(1-\epsilon)\tau\}$\label{line:complete}
\end{algorithmic}
\end{algorithm}

\begin{theorem}
    \label{theorem:stochastic}
   With probability at least $1-\frac{1}{n^2}$, Algorithm \ref{alg:stoc_cover}
   outputs a solution $S$ that satisfies a $(\lceil\ln(3/\epsilon)\rceil,1-\epsilon)$-bicriteria approximation guarantee in $O(n\ln^2(3/\epsilon)\ln(|OPT|))$ queries of $f$.
\end{theorem}

TODO: Need to make sure $f$ is cut off at $\tau$ everywhere because of Markov.
Before the proof of Theorem \ref{theorem:stochastic}, we prove two needed lemmas.

\begin{lemma}
\label{lem:sgc_expection}
    Once $r$ reaches $\lceil\ln(3/\epsilon)|OPT|\rceil$, for all $i$
    \begin{align*}
    \mathbb{E}f_\tau(S_i) &\geq\left(1-\frac{\epsilon}{2}\right)\tau.
    \end{align*}
\end{lemma}
\begin{proof}
    Consider any iteration of the while loop in \sgbi where $r<\lceil\ln(3/\epsilon)|OPT|\rceil$. Then
    \begin{align*}
        |R|\geq \frac{n}{|OPT|}\ln(3/\epsilon).
    \end{align*}
    Therefore, for each of the sampled $R$,
    \begin{align*}
        P(R\cap OPT = \emptyset) = (1-|OPT|/n)^{|R|}\leq (1-|OPT|/n)^{n\ln(3/\epsilon)/|OPT|}
        \leq \epsilon/3.
    \end{align*}
    In addition, for each set $S_i$ which is adding $u_i$,
    \begin{align*}
        \mathbb{E}[\Delta f(S_i, u_i)| R\cap OPT \neq\emptyset]\geq \frac{1}{|OPT|}\sum_{o\in OPT}\Delta f(S_i,o) \geq \frac{1}{|OPT|}\sum_{o\in OPT}(\tau - f(S_i)).
    \end{align*}
    Altogether we have that once $r$ reaches $\lceil\ln(3/\epsilon)|OPT|\rceil$, for all $i$,
    \begin{align*}
        \mathbb{E}[f(S_i)]\geq (1-\epsilon/2)\tau.
    \end{align*}
\end{proof}

\begin{lemma}
\label{lem:sgc_high_prob}
    With probability at least $1-\delta$, once $r$ reaches $\lceil\ln(3/\epsilon)|OPT|\rceil$, we have that $\max_{i}f(S_i)\geq(1-\epsilon)\tau$.
\end{lemma}
\begin{proof}
    Since $f_\tau(S)=\min\{f(S),\tau\}$, we have that $\tau-f_\tau(S)\in[0,\tau]$ for any $S\in  U$. By applying the Markov's inequality, we have that
    \begin{align*}
        P(\tau-f_\tau(S_j)\geq 2\mathbb{E}(\tau-f_\tau(S_j))\leq\frac{1}{2}
    \end{align*}
From Lemma \ref{lem:sgc_expection}, we have $\mathbb{E}(\tau-f_\tau(S_j))\leq\frac{\epsilon\tau}{2}$. Then 
\begin{align*}
    P(f_\tau(S_j)\leq(1-\epsilon)\tau)&=P(\tau-f_\tau(S_j)\geq\epsilon\tau)\\
    &\leq P(\tau-f_\tau(S_j)\geq 2\mathbb{E}(\tau-f_\tau(S_j)))\\
    &\leq\frac{1}{2}.
\end{align*}
Thus we have
\begin{align*}
    P(\max_j f_\tau(S_j)>(1-\epsilon)\tau)&=1-P( f_\tau(S_j)\leq(1-\epsilon)\tau,\forall j)\\
    &=1- P( f_\tau(S_1)\leq(1-\epsilon)\tau)^{\ln(1/\delta)/\ln(2)}\\
    &\geq1-\left(\frac{1}{2}\right)^{\ln(1/\delta)/\ln(2)}\geq1-\delta.
\end{align*}
\end{proof}
%  By Hoeffding's inequality, we have that with probability $1-\frac{1}{n^2}$, 
% \begin{align}
% \frac{\sum_{j=1}^Nf_\tau(S^{(j)})}{N}\geq\mathbb{E}f_\tau(S^{(1)}_{r_0})-\epsilon\tau/3
% \end{align}

Now, we can prove Theorem \ref{theorem:stochastic}.
\begin{proof}
    From Lemma \ref{lem:sgc_high_prob}, the algorithm stops before $r$ reaches $\lceil\ln(3/\epsilon)|OPT|\rceil$ with probability at least $1-\delta$, so the size of output set satisfies that $|S|\leq \lceil\ln(3/\epsilon)\cdot |OPT|\rceil$. The number of queries is upper bounded as
    $$\ln(1/\delta)/\ln(2)\sum_{i=1}^{|OPT|}\frac{n}{i}\ln^2(3/\epsilon)
    =O(n\ln^2(3/\epsilon)\ln(|OPT|)).$$
\end{proof}

\end{subsubsection}
\end{subsection}

==> Sections/Old/ProblemSetup.tex <==
\section{Problem Statement and Preliminaries}
In this section, we present the problem setup 
and notations used in this paper. Throughout this paper, we consider set functions from ground set $U$ to $\mathbb{R}$.   
For any set function  $f:2^U\to\mathbb{R}$, and $\forall i\in U$, $A\subseteq U$, denote the marginal gain of adding element $i$ to set $A$ as $\Delta(A, i) $, i.e., $\Delta(A, i)=f(A\cup i)-f(A)$.                          
\subsection{Submodular Maximization}
\begin{definition}
    A function $f:2^U\to\mathbb{R}$ is  submodular  if it satisfies
    $\forall A\subseteq B\subseteq U$ and $i\in U$, we have that $\Delta f(A,i)\geq\Delta f(B,i)$. 
  Furthermore, if the function also satisfies $\forall A,B\subseteq U$, if $A\subseteq B$, then $f(A)\leq f(B)$, then $f$ is monotone.    
\end{definition}

\subsection{Regularized Objective}
\begin{definition}[The Knapsack Constrained Regularized Submodular Maximization Problem (KRSM)] Let $f:2^U\to\mathbb{R}$ be a monotone submodular function defined on subsets of ground set U of size $n$.
    $c,g:U\to\mathbb{R}_{>0}$ be modular function over subsets of $U$. Then the optimization problem is, given budget $\kappa\in\mathbb{R}_{\geq 0}$, find
    $$\argmax\{f(X)- g(X):c(X)\leq \kappa\}.$$
\end{definition}
\begin{definition}
An $(\alpha,\beta,\gamma)$-multicriteria approximation algorithm for KRSM produces a solution $S$ such that 
$f(S)-g(S)\geq\alpha\max_{X\in U ,c(X)\leq\kappa}\{f(X)-\gamma g(X)\}$ and $c(S)\leq\beta\kappa$ where $S^*$ is the optimal solution.
\end{definition}
\paragraph{Notations.} In this paper, we denote the optimal solution for any discrete optimization problem $\max_{S\in\mathcal{I}}f(S)$ as $S^*$. Denote the upper bound and lower bound of the cost function $c(u)$ as $c_{\text{min}}$ and $c_{\text{max}}$ separately, i.e., $\cmin\leq c(u)\leq\cmax$, $\forall u\in U$. 
Furthermore, when the cost function is uniform unit cost, i.e., $c(u)=1$ for any $u\in U$, we have that $\cmin=\cmax=1$. 
The Knapsack constraint is then reduced to cardinality constraint. 

==> Sections/Old/StochasticGreedy.tex <==
We consider here the special case of \ksm where $c(x)=1$ for all $x\in U$, called \csml (\csm).

\begin{algorithm}
\label{alg:sg}
\begin{algorithmic}[1]

\Procedure{\sg}{$\epsilon$}
  \State $S\gets\emptyset$
  \While{$|S|<\ln(1/\epsilon)\kappa$}
    \State $R\gets$ sample $\frac{n}{\kappa}\ln(1/\delta)$ elements from $U$
    \State $u\gets\argmax_{x\in R}\Delta f(S,x)$
  \EndWhile
  \State \textbf{return} $S$
\EndProcedure

\end{algorithmic}
\end{algorithm}

\begin{theorem}
    \sg produces a solution with $(1-\delta-\epsilon,\ln(1/\delta))$-bicriteria approximation guarantee to \csm, where the $1-\delta-\epsilon$ holds in expectation, in $\ln(1/\delta)\ln(1/\epsilon)n$ queries of $f$.
\end{theorem}

\begin{proof}
Here we denote the set $S$ we obtained before the $i$-th step as $S_i$, the item to be added to set $S$ at step $i$ is $u_i$ and the sampled set $R$ is $R_i$. Consider for any item $u\in R_i\cap S^*$, we have that
\begin{align*}
    \Delta f(S_i,u_i)\geq f(S_i,u)
\end{align*}
It follows that
\begin{align*}
    \Delta f(S_i,u_i)\geq\frac{1}{|R_i\cap S^*|}\sum_{u\in R_i\cap S^*} f(S_i,u).
\end{align*}
Here we use similar approaches as in \cite{mirzasoleiman2015lazier}. Since $R_i$ is randomly chosen, we have that in expectation
\begin{align}
\label{eqn:stoc_greedy}
    \mE[\Delta f(S_i,u_i)|S_i]\geq\textbf{Pr}(R_i\cap S^*\neq \emptyset)\frac{1}{\kappa}\sum_{u\in S^*} f(S_i,u).
\end{align}
The probability $\textbf{Pr}(R_i\cap S^*\neq \emptyset)$ can be lower bounded as
\begin{align}
\label{eqn:prob_of_intersection}
    \textbf{Pr}(R_i\cap S^*\neq \emptyset)&=1-\textbf{Pr}(R_i\cap S^*= \emptyset)\notag\\
    &=1-\frac{\binom{n-s}{\kappa }}{\binom{n}{\kappa }}\notag\\
    &\geq1-(\frac{n-s}{n})^{\kappa }\notag\\
    &\geq1-\delta ,
\end{align}
where the last inequality comes from the fact that $(1-\frac{1}{x})^x\leq e^{-1}$. 
By submodularity, we have 
\begin{align}
\label{eqn:submodularity_CSM}
   \sum_{u\in S^*} \Delta f(S_i,u)\geq f(S^*)-f(S_i).
\end{align}
Plug Equations (\ref{eqn:prob_of_intersection}) and (\ref{eqn:submodularity_CSM}) into (\ref{eqn:stoc_greedy}) yields that
\begin{align}
    \mE[\Delta f(S_i,u_i)|S_i]\geq \frac{1-\delta }{\kappa }(f(S^*)-f(S_i)).
\end{align}
Therefore,
\begin{align*}
    \mE[ f(S_{i+1})|S_i]\geq \frac{1-\delta }{\kappa }f(S^*)+(1-\frac{1-\delta }{\kappa })f(S_i)).
\end{align*}
By induction and by taking expectation over $S_i$, we can get that at the last iteration
\begin{align*}
    \mE[ f(S_{T})]&\geq \frac{1-\delta }{\kappa }\sum_{i=0}^{T-1}(1-\frac{1-\delta }{\kappa })^if(S^*)\\
    &\geq 
    \{1-(1-\frac{1-\delta }{\kappa })^T\}f(S^*)\\
    &\geq 
    (1-\epsilon^{1-\delta})f(S^*)\geq  
    (1-\epsilon-\delta)f(S^*),
\end{align*}
where in the last inequality, we use the fact that $T$ is the number of iterations and is thus equal to the cardinality of set $S$, which is $\ln(1/\epsilon)\kappa$.
\end{proof}

==> Sections/Old/Streaming.tex <==

\begin{algorithm}
\label{alg:stream}
\begin{algorithmic}[1]

\Procedure{\stream}{$\epsilon,OPT$}
  \State $S\gets\emptyset$
  \While{$u$ arrives from the stream}
    \If{$c(S\cup \{u\})\leq \kappa/\epsilon$ and $\Delta f(S,u)/c(u)\geq \epsilon OPT/\kappa$}
        \State $S\gets S\cup\{u\}$
    \EndIf
  \EndWhile
  \State \textbf{return} $S$
\EndProcedure

\end{algorithmic}
\end{algorithm}

The $OPT$ in \stream refers to the optimal solution of \ksm, i.e. $OPT=\max\{f(X):|X|\leq\kappa\}$. Can do guessing in parallel in order to find the correct one.


% In the theorem below, we present result for KSM that achieves best approximation guarantee with multilinear extension. 
% \begin{definition}
%     Any submodular function $f:2^U\to\mathbb{R}$  with a universe $U$ of size $n$ can be extended as a continuous function $F:[0,1]^n\to\mathbb{R}$. More specificly,
%     \begin{align}
%         F(\textbf{x})=\sum_{S\in U}f(S)\prod_{i\in S}x_i\prod_{i\notin S}(1-x_i).
%     \end{align}
    
% \end{definition}
% The multilinear relaxation  of KSM problem is then $\max\{F(\textbf{x}):\textbf{c}^Tx\leq\kappa\}$.
% \begin{theorem}
%     The continuous greedy algorithm for the problem $\max\{F(\textbf{x}):\textbf{c}^Tx\leq\kappa\}$ would produce a solution with $(1-\epsilon,\ln(1/\epsilon))$ approximation guarantee.
% \end{theorem}
% \begin{proof}
    
% \end{proof}

==> Sections/Old/TheoreticalCover.tex <==
\section{Algorithms for \ksc}

\subsection{Converting Algorithms for \ksm}
\begin{lemma}
\label{lem:dual_opt}
Denote 
% the optimal solution set for KSM($\kappa$) as $M_{\kappa}^*$, and 
the optimal value for KSC($\tau$) as $OPT_\tau$. Then we have that any optimal solution for problem KSM($OPT_\tau$) is optimal for KSC($\tau$). Besides, the optimal value of KSM($OPT_\tau$) is no less than a $\tau$.
\end{lemma}
\begin{proof}
For any $S^*\in\argmax\{f(X): c(X)\leq OPT_\tau\}$, we have that $c(S^*)\leq OPT_\tau$. Suppose $S^*_\tau$ is an optimal solution for KSC($\tau$), then we have that $c(S^*_\tau)= OPT_\tau$. It implies that $S^*_\tau$ is feasible for KSM($OPT_\tau$). Thus we have $f(S^*)\geq f(S^*_\tau)\geq \tau$.

%we can see that $S_{\tau}^*$ is feasible. Thus we only need to prove the optimality. For any set $X\in U$ such that $c(X)\leq c(S^*_{\tau})$, since $S_{\tau}^*$ is optimal for $\argmin\{c(X): f(X)\geq \tau\}$, we can get $f(X)\leq \tau$. Since $f(S_{\tau}^*)\geq \tau$, $f(X)\leq \tau\leq f(S_{\tau}^*)$.

\end{proof}

% \begin{corollary}
%     Let $C$ be a constant such that $OPT_\tau\leq C\leq(1+\delta)OPT_\tau$. 
%     For any $(\alpha,\beta)$-bicriteria algorithm taking $C$ as an input would produce a set $S$ that achieves an $(\beta,(1+\delta)\alpha)$-approximation guarantee.
% \end{corollary}
% \begin{proof}
    
% \end{proof}
\begin{theorem}
    Any deterministic $(\alpha,\beta)$-bicriteria approximation algorithm for \ksm that runs in time $\mathcal{T}(n)$ can be converted into a $(\beta,\alpha)$-bicriteria approximation algorithm for \ksc that runs in time $O(\ln(n)\mathcal{T}(n))$.
\end{theorem}
\begin{algorithm}
% \label{alg:sg}
\begin{algorithmic}[1]

\Procedure{\texttt{KSC-Sto}}{$\tau$}
  \State {\bfseries{Input: }$\tau$, $\delta\in(0,1)$, $\epsilon$}
  \State{ $B\gets 0$, $r\gets 0$, $N\gets\frac{\log n}{2\epsilon^2}$}
  \While{$B<\alpha\tau-\epsilon\tau$}
    \State $C_r=(1+\delta)^rc_{min}$
    \For{$i=1$ \textbf{to} $N$}
        \State {$S^{(i)}_r\gets$\texttt{KSM-Sto}($f_\tau, C_r$)}
      \EndFor
      \State $B\gets\frac{\sum_{i=1}^Nf_\tau(S^{(i)}_r)}{N}$
     \State{$S\gets\argmax\{f(S_{r}^{(i)})\}$}
      \State $r\gets r+1$
  \EndWhile
  \State \textbf{return} $S$
\EndProcedure

\end{algorithmic}
\end{algorithm}
\begin{theorem}
    Any randomized $(\alpha,\beta)$-bicriteria approximation algorithm for \ksm that runs in time $\mathcal{T}(n)$ where $\alpha$ holds only in expectation can be converted into a $(\beta,\alpha)$-bicriteria approximation algorithm for \ksc that runs in time $O(\ln^2(n)\mathcal{T}(n))$ where $\alpha$ holds with high probability.
\end{theorem}
\begin{proof}
Here we denote 
% the random algorithm for the KSC($\tau$) problem as \texttt{KSC-Sto}($\tau$), and 
the algorithm for the KSM($\kappa$) problem as \texttt{KSM-Sto}($f,\kappa$). The optimal solution for KSC($\tau$) as $S^*_\tau$. Throughout the algorithm, we use the truncated version $f_\tau$ to replace the submodular function $f$, $f_\tau(S)=\min\{\tau,f(S)\}$.
%$\tau$ and $\kappa$ are the corresponding parameters of the constraints. 
% For notation simplicity, we further denote that the optimal solution for KSC($\tau$) as $S_{\tau}^*$, and the optimal solution for KSM($\kappa$) problem as $M_{\kappa}^*$. 
In the algorithm \texttt{KSC-Sto}($\tau$), $C_r$ is the guess of OPT. The output set $S_r^{(i)}$ of \texttt{KSM-Sto}($f_\tau,C_r$) would satisfy the bicriteria approximation guarantee that
\begin{align}
    \mE f_\tau(S_r^{(i)})&\geq\alpha\max\{f_\tau(S):c(S)\leq C_r\}\notag\\
    c(S_r^{(i)})&\leq\beta C_r.
\end{align}
By the definition of $C_r$, we have that 
 $\exists r$, such that $c(S_{\tau}^*)\leq C_r\leq(1+\epsilon)c(S_{\tau}^*)$. Then $\max\{f_\tau(S):c(S)\leq C_r\}\geq\max\{f_\tau(S):c(S)\leq c(S^*_\tau)\}$. By definition of $f_\tau$ we have $\{S:f_\tau(S)\geq\tau\}=\{S:f(S)\geq\tau\}$. Thus $S^*$ is also optimal for 
 $\argmin\{c(X): f_\tau(X)\geq \tau\}$.
 By Lemma \ref{lem:dual_opt}, we have
\begin{align}
    \mE f(S_r^{(i)})&\geq\alpha\max\{f(S):c(S)\leq c(S^*_\tau)\}\geq\alpha\tau\notag\\    
c(S_r^{(i)})&\leq(1+\delta)\beta c(S_{\tau}^*),
\end{align}
From Hoeffding's inequality, the empirical mean of $S^{(i)}_r$ would satisfy that with probability at least $1-\frac{1}{n}$,
\begin{align}
    \frac{\sum_{i=1}^Nf_\tau(S^{(i)}_r)}{N}\geq\mE f_\tau(S_r^{(1)})-\epsilon\tau\geq\alpha\tau-\epsilon\tau.
\end{align}
The algorithm stops before $c(S_{\tau}^*)\leq C_r\leq(1+\epsilon)c(S_{\tau}^*)$ with probability at least $1-\delta$. Thus the output would satisfy $c(S)\leq(1+\delta)\beta c(S^*_\tau)$. The sample complexity would be $O(\ln(n) N\mathcal{T}(n))$=$O(\ln^2(n)\mathcal{T}(n))$.
\end{proof}

\begin{algorithm}
% \label{alg:sg}
\begin{algorithmic}[1]

\Procedure{\texttt{KSC-Stream}}{$\tau$}
  \State {\bfseries{Input: }$\tau$, $\delta\in(0,1)$}
  \State{ $S_{-1}\gets\emptyset$, $r\gets-1$}
  \While{$f(S_r)<\alpha\tau$}
  \State $r\gets r+1$
  \State $C_r=(1+\delta)^rc_{min}$
        \State {$S_r\gets$\texttt{KSM-Stream}($C_r$)}
  \EndWhile
  \State \textbf{return} $S$
\EndProcedure

\end{algorithmic}
\end{algorithm}

Should talk about how you can't have a single pass cover algorithm.s

\begin{theorem}
    Any streaming $(\alpha,\beta)$-bicriteria approximation algorithm for KSM that runs in 
    $\mathcal{P}(n)$ passes and requires space usage of 
    $\mathcal{M}(n)$ can be converted into a $(\beta,\alpha)$-bicriteria approximation algorithm for KSC that runs in 
    $O((\log\frac{OPT}{\cmin})\mathcal{P}(n))$ passes and requires space usage of 
    $\mathcal{M}(n)$. Here $OPT_\tau$ is the optimal value of $KSC(\tau)$.
\end{theorem}
\begin{proof}
{\color{blue}Might need some proofs about $\cmin$ here.}  When $C_r$ increases and falls into the range that $c(S^*)\leq C_r \leq(1+\delta)c(S^*)$, we have that
\begin{align*}
    f(S_r)&\geq\alpha\max\{f(S):c(S)\leq C_r\}\\
    &\geq\alpha\max\{f(S):c(S)\leq c(S^*)\}\geq\alpha\tau,
\end{align*}
where the last inequality follows from Lemma \ref{lem:dual_opt}. Beside, we have
\begin{align*}
    c(S_r)\leq\beta C_r\leq (1+\beta)c(S^*)
\end{align*}
Define $r_0$ to be $r_0=1+\frac{\log(c(S^*)/\cmin)}{\log{1+\delta}}$. It follows that $C_{r_0}=\cmin(1+\delta)^{r_0}\geq (1+\delta)c(S^*)$. Thus the algorithm stops before $r=r_0$. 
\end{proof}
What about the distorted case?
\subsection{Converting algorithm for Regularized Objective}
In this subsection, we consider the regularized submodular optimization problem.
\begin{algorithm}
% \label{alg:sg}
\begin{algorithmic}[1]

\Procedure{\texttt{KRSC-Alg}}{$\tau$}
  \State {\bfseries{Input: }$\tau$, $\delta\in(0,1)$, }
  \State{ $S_{-1}\gets \emptyset$, $r\gets -1$}
  \While{$f(S_{r})-\frac{1}{\gamma}g(S_{r})<\alpha\tau$}
  \State $r\gets r+1$
    \State $C_r=(1+\delta)^rc_{min}$ 
        \State {$S_r\gets$\texttt{KRSM-Sto}($f,\frac{1}{\gamma}g, C_r$)}
     % \State{$S\gets S_r$}
      
  \EndWhile
  \State \textbf{return} $S_{r}$
\EndProcedure

\end{algorithmic}
\end{algorithm}
%\input{Sections/DistortedGreedy2.tex}
\begin{theorem}
    Any deterministic $(\alpha,\beta,\gamma)$- multicriteria algorithm for KRSM that runs in time $\mathcal{T}(n)$ could be converted into an algorithm for KRSC that outputs a set satisfying
    \begin{align*}
    &c(S)\leq\beta(1+\delta) c(S^*)\notag\\
        &f(S)- \frac{1}
        {\gamma}g(S)\geq\alpha\tau.
    \end{align*}
 The runtime is then $O(\ln(n)\mathcal{T}(n))$.
\end{theorem}
\begin{proof}
    Denote $S^*=\argmax_{S\in U,f(S)-g(S)\geq\tau}c(S)$, and that $g'(S)=\frac{1}{\gamma}g(S)$.
    When $C_r$ increases and falls into the range that $c(S^*)\leq C_r \leq(1+\delta)c(S^*)$, we have that \texttt{KRSM-Sto}($f,\frac{1}{\gamma}g, C_r$) would produce a solution such that
    \begin{align*}
        f(S_r)-g'(S_r)&\geq\alpha\max_{c(X)\leq C_r}(f(X)-tg'(X))\\
&\geq\alpha\max_{c(X)\leq c(S^*)}(f(X)-tg'(X))\\
&\geq\alpha\max_{c(X)\leq c(S^*)}(f(X)-g(X))\\
&\geq\alpha\tau,
    \end{align*}
    where the last inequality follows from Lemma \ref{lem:dual_opt}.
    Besides, we also have that $c(S_r)\leq\beta C_r\leq\beta(1+\delta)c(S^*)$. Thus the algorithm stops before $c(S^*)\leq C_r \leq(1+\delta)c(S^*)$.
\end{proof}
\subsection{The Case Where $\tau=\max\{f(Y): Y\subseteq U\}$}
{\color{blue} In this section, we consider the case where we wish to set 
$\tau=\max\{f(Y): Y\subseteq U\}$ but the value of $\tau$ is not necessarily known.}

==> Sections/Old/TheoreticalMax.tex <==
\section{Algorithms for \ksm}
\label{section:ksm}
Need to discuss the standard greedy algorithm here. May have already been proven?

TODO: Tightness of the logarithmic factor? Tightness of the streaming guarantee as well?

\subsection{Monotone and Non-Negative Objectives}
First we present a tightness example which shows that the greedy algorithm bicriteria doesn't do better than
    $(1-\epsilon,\log_{1-1/k}(\epsilon)/k)$.
\begin{theorem}
    (Needs to be written more clearly)
    Tight example that the greedy algorithm bicriteria doesn't do better than
    $(1-\epsilon,\log_{1-1/k}(\epsilon)/k)$.
\end{theorem}
\begin{proof}
    Instance of set cover as follows.
    Let the cardinality constraint be $k$.
    The elements needing to be covered form $k$ groups of size $\ell$ each.
    The sets that cover the elements are $S_1,...,S_k$, where $S_i$ covers the $i$th group, and then sets $A_i$ defined inductively as follows: $A_1$ covers the first $\ell/k$ elements from each group, $A_2$ covers the next $(1-1/k)\ell/k$ elements from each group,
    $A_3$ the next $(1-1/k)^2\ell/k$ from each group, and so on.
    The optimal solution to the instance is picking $S_1,...,S_k$, but the greedy will choose $A_1,A_2,...$.
    In order to have $f(\{A_1,A_2,...\})\geq (1-\epsilon)f(OPT)$, exactly $\log_{1-1/k}(\epsilon)$ of the sets $A_1,A_2,...$
    must be chosen.
\end{proof}
\paragraph{Remark. }Notice that here $\lim_{k\rightarrow\infty}\log_{1-1/k}(\epsilon)/k=\log1/\epsilon$, so the tight example would produce an approximation guarantee of $(1-\epsilon,\log1/\epsilon)$ when $k$ goes to infinity.

\input{Sections/Streaming.tex}

\subsection{Regularized Objectives}

\input{Sections/DistortedGreedy.tex}

\begin{theorem}
    Distorted stochastic greedy.
\end{theorem}

\input{Sections/DistortedStreaming.tex}

\subsection{Non-Negative Objectives}
This will include my results from my AISTATS paper.

Give example about how several common algorithms cannot be turned into bicriteria (e.g. random greedy).

Hardness result.

==> graphs/greedy.tex <==

\begin{tikzpicture}[scale=0.9]
\draw (0,0) -- (1.75,0);

\node at (0,0.5) {\small$0$};
\draw (0,-0.2) -- (0,0.2);

\draw [WildStrawberry,thick,-{Latex[length=2mm,width=2mm]}] (0,-0.25) to [out=-60,in=-135] (1.5,-0.25);

\node at (0.75,-0.85) {\small  $R=U$};

\node at (1.5,0.5) {\small$\ln(3/\epsilon)$};
\draw (1.5,-0.2) -- (1.5,0.2);

\node at (2.25,0) {.....};
\draw (2.75,0) -- (10,0);

\draw [WildStrawberry,thick,-{Latex[length=2mm,width=2mm]}] (2,-0.25) to [out=-60,in=-135] (4,-0.25);

\node at (2.25,-1) {\small add $a_2$};


\node at (4,0.5) {\small$2\ln(3/\epsilon)$};
\draw (4,-0.2) -- (4,0.2);

\draw [WildStrawberry,thick,-{Latex[length=2mm,width=2mm]}] (4,-0.25) to [out=-60,in=-135] (7,-0.25);

\node at (4.4,-1) {\small add $a_3$};


\node at (7,0.5) {\small$4\ln(3/\epsilon)$};
\draw (7,-0.2) -- (7,0.2);


\draw [WildStrawberry,thick,-{Latex[length=2mm,width=2mm]}] (7,-0.25) to [out=-60,in=-135] (10,-0.25);

\node at (7.8,-0.8) {\small add $4\ln(3/\epsilon)$};


\node at (10,0.5) {\small$8\ln(3/\epsilon)$};
\draw (10,-0.2) -- (10,0.2);

\node at (11,0) {.....};

\node at (12,-0.5) {\small$2\ln(3/\epsilon)|OPT|$};
\draw (12,-0.2) -- (12,0.2);
\end{tikzpicture}


==> graphs/stream.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}[scale=0.25]

\draw (17,0) ellipse (3cm and 4cm);
\draw [cyan, fill=cyan] (18,-0.5) circle [radius=0.25];
\draw [cyan, fill=cyan] (19,1.5) circle [radius=0.25];
\draw [cyan, fill=cyan] (17.5,1) circle [radius=0.25];
\draw [cyan, fill=cyan] (16,-3) circle [radius=0.25];
\draw [cyan, fill=cyan] (15.5,-1.5) circle [radius=0.25];
\draw (17,-5.5) node {\small$S_{2/\epsilon}$};

\draw (10,0) ellipse (3cm and 4cm);
\draw [cyan, fill=cyan] (9,2) circle [radius=0.25];
\draw [cyan, fill=cyan] (7.5,0.5) circle [radius=0.25];
\draw [cyan, fill=cyan] (12.5,1.5) circle [radius=0.25];
\draw [cyan, fill=cyan] (10.5,-1) circle [radius=0.25];
\draw [cyan, fill=cyan] (10,-3) circle [radius=0.25];
\draw [cyan, fill=cyan] (8.5,-1.5) circle [radius=0.25];
\draw (10,-5.5) node {\small$S_{2/\epsilon-1}$};


\draw (0,0) ellipse (3cm and 4cm);
\draw [cyan, fill=cyan] (-1,-2) circle [radius=0.25];
\draw [cyan, fill=cyan] (-2.5,0) circle [radius=0.25];
\draw [cyan, fill=cyan] (2.5,-0.5) circle [radius=0.25];
\draw [cyan, fill=cyan] (0,-1) circle [radius=0.25];
\draw [cyan, fill=cyan] (0,-3) circle [radius=0.25];
\draw [cyan, fill=cyan] (-1.5,-1.5) circle [radius=0.25];
\draw (0,-5.5) node {\small$S_1$};

\draw [dotted, thick] (6,0) to (4,0);

\draw [WildStrawberry,thick,-{Latex[length=2mm,width=2mm]}] (24,0) to (21,0);
\draw [cyan, fill=cyan] (25,0) circle [radius=0.25];
\draw [cyan, fill=cyan] (26,0) circle [radius=0.25];
\draw [cyan, fill=cyan] (27,0) circle [radius=0.25];
\draw [cyan, fill=cyan] (28,0) circle [radius=0.25];
\draw [dotted, thick] (30.5,0) to (29.5,0);
\draw node at (27,-1.5) {\small Stream of $U$};

\end{tikzpicture}
\caption{An illustration of \filt. Each blue dot represents an element of $U$.
As elements of $U$ arrive,
and each element is either discarded or stored in at most one of
the disjoint sets $S_1,...,S_{2/\epsilon}$.
%An element $u$ is stored
%in a set $S_j$ if both of the following are true:
%(i) $u$ has sufficiently low cost;
%(ii) adding $u$ is sufficiently beneficial to increasing
%the $f$ value of $S_j$.
%$\Delta f(S_j,u)\geq w(u)\epsilon \tau/(2 \guess)$.
%If no such $S_j$ exists, $u$ is discarded.
%If the total cost of one of the disjoint sets gets too high
%before all elements of $U$ have been read in, then \stream stops reading in elements.
At the completion of reading elements from the stream,
\filt runs submodular maximization on the union of the disjoint sets.}
\label{fig:stream}
\end{figure}

